Robust Hierarchical Patterns for identifying MDD patients: A Multisite Study

Many supervised machine learning frameworks have been proposed for disease classification using functional magnetic resonance imaging (fMRI) data, producing important biomarkers. More recently, data pooling has flourished, making the result generalizable across a large population. But, this success depends on the population diversity and variability introduced due to the pooling of the data that is not a primary research interest. Here, we look at hierarchical Sparse Connectivity Patterns (hSCPs) as biomarkers for major depressive disorder (MDD). We propose a novel model based on hSCPs to predict MDD patients from functional connectivity matrices extracted from resting-state fMRI data. Our model consists of three coupled terms. The first term decomposes connectivity matrices into hierarchical low-rank sparse components corresponding to synchronous patterns across the human brain. These components are then combined via patient-specific weights capturing heterogeneity in the data. The second term is a classification loss that uses the patient-specific weights to classify MDD patients from healthy ones. Both of these terms are combined with the third term, a robustness loss function to improve the reproducibility of hSCPs. This reduces the variability introduced due to site and population diversity (age and sex) on the predictive accuracy and pattern stability in a large dataset pooled from five different sites. Our results show the impact of diversity on prediction performance. Our model can reduce diversity and improve the predictive and generalizing capability of the components. Finally, our results show that our proposed model can robustly identify clinically relevant patterns characteristic of MDD with high reproducibility.

==> Figures/scp.tex <==
\begin{figure}
  \centering
  \hspace{-1.8em} $\mathbf{\Theta}^i \hspace{1.8em}\approx \hspace{1.8em} \Lambda^i_1 \mathbf{w}_1\mathbf{w}_1^\top \hspace{1em} + \hspace{1em} \Lambda^i_1 \mathbf{w}_2\mathbf{w}_2^\top \hspace{1em} + \hspace{1em} \Lambda^i_1 \mathbf{w}_3\mathbf{w}_3^\top  $ \\
  
  \vspace{0.5em}
\includegraphics[scale=0.1, valign=c]{Figures/c_matrix.png}
  % Top images 
  \hspace{3.5em}
  $\mathbf{w}_1 \rightarrow$ \hspace{-0.6em}
  \includegraphics[trim={3cm 1cm 2cm 1cm},clip,scale=0.15, valign=c]{Figures/Images/sahoo21.png}
  \hspace{0.5em}$\mathbf{w}_2 \rightarrow$ \hspace{-0.6em}
  \includegraphics[trim={3cm 1cm 2cm 1cm},clip,scale=0.15, valign=c]{Figures/Images/sahoo22.png}
   \hspace{0.6em}$\mathbf{w}_3 \rightarrow$ \hspace{-0.6em}
  \includegraphics[trim={3cm 1cm 2cm 1cm},clip,scale=0.15, valign=c]{Figures/Images/sahoo23.png}

  \medskip
  \caption{Schematic illustrating SCP where $\mathbf{\Theta}^i$ is a subject specific correlation matrix which is approximated by non-negative sum of sparse rank one matrices.}
    \label{fig:ex_scp}
\end{figure}

==> Tables/detailed_dataset_table.tex <==
\begin{table}[t]
 \caption{Summary characteristics of the real dataset.}
 \label{tbl:summary}
\centering
\begin{tabular}{ lcccc }
 \hline

Data Sites  & Participants & \% of Females & Age Range (Median) & \% of MDD \\
 \hline
 EMBARC-CU   & $89$ & $67.4$ & $[18,64](30)$  & $88.6$\\
 EMBARC-MG  & $62$  & $58.0$ & $[18,65](28)$ & $83.8$\\
 EMBARC-TX   & $108$  & $65.7$ & $[19,65](43)$ & $89.8$ \\
 EMBARC-UM   & $69$  & $71.0$ & $[18,65](31)$ & $85.5$\\
 Oxford  & $70$& $59.4$ & $[19,61](28)$ & $55.0$\\
SCU   & $70$ & $52.8$ & $[16,60](28.5)$&  $42.8$ \\
SNAP    & $110$ & $64.5$ & $[19,58](28.5)$&  $50.0$\\
STRADL    & $1079$ & $59.3$ & $[26,84](61)$&  $30.0$\\
 \hline

\end{tabular}

\end{table}
%EMBARC 329

==> dataset_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ llllll }
 \hline

Data Sites & No. of Participants  & Age Range (Median) & Similarity with pooled components\\
 \hline
 BLSA-3T    & $784$  & $[22,95](68)$ & $0.6136$\\
 CARDIA\_1   & $199$   & $[42,61](52)$ & $0.5902$\\
 CARDIA\_3   & $321$  & $[43,61](52)$ & $0.5636$\\
 CARDIA\_4   & $278$   & $[43,62](52)$ & $0.5470$\\
 UKBB  & $2023$&  $[45,79](63)$ & $0.6518$\\
OASIS    & $847$ &$[42.6,97](70)$ & $0.6316$\\
ADC   & $279$ &  $[23,95](70)$ & $0.5264$\\
 \hline

\end{tabular}
 \caption{Summary characteristics of the datasets. Last column shows similarity of the components derived from individual sites with the components derived from the pooled dataset. We can see that sites having larger sample size have more similarity with the components derived from the pooled dataset. \textbf{Todo}: Show age distribution}
 \label{fig:summary}
\end{table}


==> explanation.tex <==
We are working on a hypothetical scenario here. Let there be $4$ networks (some group of regions) A, B, C and D. A is positively correlated with B and negatively correlated with C. C does not have correlation with B. D is only positively correlated with C. So we have below correlation matrix representing the above information:

\begin{equation}
\begin{pmatrix} 1 & 1 & -1 & 0\\ 1 & 1 & 0 & 0 \\ -1 & 0 & 1 & 1 \\ 0 & 0 & 1 & 1\end{pmatrix}  = 
\end{equation}

The information described above can be written in vectors/patterns form as:

\begin{equation}
\begin{pmatrix} 1 & 1 & -1 & 0\\ 1 & 1 & 0 & 0 \\ -1 & 0 & 1 & 1 \\ 0 & 0 & 1 & 1\end{pmatrix}  \approx 
x_1\begin{pmatrix} 1 \\ 1 \\ 0 \\ 0\end{pmatrix} \begin{pmatrix} 1 & 1 & 0 & 0\end{pmatrix} +
x_2\begin{pmatrix} 1 \\ 0 \\ -1 \\ 0\end{pmatrix} \begin{pmatrix} 1 & 0 & -1 & 0\end{pmatrix} + 
x_2\begin{pmatrix} 0 \\ 0 \\ 1 \\ 1\end{pmatrix} \begin{pmatrix} 0 & 0 & 1 & 1\end{pmatrix} 
\end{equation}

First term in RHS depicts that A is correlated with B but since A and B jointly together does not have any correlation, the other terms are zero and only 1st and 2nd term are 1. Similar second terms depicts that A is negatively correlated with C. We can flip the signs here, but the inference will remain the same. Third term shows that C and D are positively correlated. Right hand side of the above term can be expanded and we get:

\begin{align}
    RHS & = x_1\begin{pmatrix} 1 \\ 1 \\ 0 \\ 0\end{pmatrix} \begin{pmatrix} 1 & 1 & 0 & 0\end{pmatrix} +
x_2\begin{pmatrix} 1 \\ 0 \\ -1 \\ 0\end{pmatrix} \begin{pmatrix} 1 & 0 & -1 & 0\end{pmatrix} + 
x_2\begin{pmatrix} 0 \\ 0 \\ 1 \\ 1\end{pmatrix} \begin{pmatrix} 0 & 0 & 1 & 1\end{pmatrix} \\
& = x_1\begin{pmatrix} 1 & 1 & 0 & 0\\ 1 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0\end{pmatrix}  + x_2\begin{pmatrix} 1 & 0 & -1 & 0\\ 0 & 0 & 0 & 0 \\ -1 & 0 & 1 & 0 \\ 0 & 0 & 0 & 0\end{pmatrix}  + x_3\begin{pmatrix} 0 & 0 & 0 & 0\\ 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 1 \\ 0 & 0 & 1 & 1\end{pmatrix} 
& = \begin{pmatrix} x_1+x_2 & 1 & 0 & 0\\ 1 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0\end{pmatrix} 
\end{align}

==> new_dataset_table.tex <==
\begin{table}[t!]
 \caption{Summary characteristics and age range along with the median is shown for each data site.}
 \label{tbl:summ}
\centering
\begin{minipage}[t]{0.45\linewidth}
\begin{tabular}[t]{ ccc}
 \hline

Data Site & Participants  & Age Range \\
 \hline
 BLSA-3T    & $784$  & $[22,95](68)$ \\
 CARDIA\_1   & $199$   & $[42,61](52)$ \\
 CARDIA\_3   & $321$  & $[43,61](52)$ \\
 CARDIA\_4   & $278$   & $[43,62](52)$ \\
 \hline

\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth}
\begin{tabular}[t]{ ccc }
 \hline

Data Site & Participants  & Age Range\\
 \hline
UKBB  & $2023$&  $[45,79](63)$\\
OASIS    & $847$ &$[42.6,97](70)$ \\
ADC   & $279$ &  $[23,95](70)$ \\
 \hline

\end{tabular}
\end{minipage}

\end{table}

==> review.tex <==
What is the unqiueness of our papper?
Objective and focus of our review?
1) using GANs; 2) provide disease/pathology insights
But what if there are papers which just provide methodological insight i.e. if their focus is only on methods and improving the accuracy
Have we identified sufficient future directions for this field? Are we in a position to summarize the challenges, limitations and issues in the field? 

\cite{mirakhorli2020new}
The paper uses resting-state fMRI data to identify abnormal changes in the brain due to disorders. The method is based on the idea that disorder changes the functional connectivity of the human brain and uses this idea to understand the changes in the human brain. They use functional connectivity to represent the human brain by a graph using functional connectivity, and then a use them in graph deep learning model is used to learn structures differentiating AD subjects from healthy ones. The model is built using Variational Graph Autoencoder (VGAE) & GAN consisting of several GCNN based on the architecture defined in \cite{yang2019conditional}. 

They employed a graph embedding model for converting graph data into a low dimensional space, and used graph matching and partial graph completion problems \cite{verma2018feastnet} to identify the abnormal parts of the input graphs.

The experiments were performed on 192 subjects from pre-processing ADNI dataset, including 96 AD, 48 normal control and 48 MCI. The results indicate that abnormal connections of the Frontal Gyrus and Precentral Gyrus with other regions can have a high percentage of AD risk in the early stages and fall into the effective biomarkers category. In addition to these regions, they also found the Olfactory cortex (OLF), Supplementary Motor Area (SMA), and Rolandic Opercular (ROL) to have a high contribution to classify MCI.

% Can we exclude it? Problems- No quantitative assessment and comparison with other methods. The only comparison they have with some non state of the art methods and the sample size is also different. Poorly written, not very detailed and information is missing.

\cite{yu2021tensorizing}
Tensorizing GAN with High-Order Pooling for Alzheimer’s Disease Assessment-

The paper proposed a deep learning based method for semi-supervised learning to utilize both labeled and unlabeled MRI images to
assess Mild Cognitive Impairment (MCI) and Alzheimer’s Disease (AD). Authors leveragedSemi-Supervised GAN (SS-GAN) \cite{radford2015unsupervised,odena2016semi} model to characterize the high-order distribution of MRI images for semi-supervised classification. The approach in the paper is different from previous GAN applications focusing on image synthesis, and image-to-image translation for AD diagnosis \cite{islam2020gan}. To tackle the problem of instability in SS-GAN, they used triple-GAN \cite{li2017triple} which is a three-player game unlike the traditional two-player model of GANs by adding auxiliary classifier based on Generator and Discriminator. Contributions-
1)Tenosrization of the three-player game is proposed to benefit from the structural information of the brain
2) As opposed to traditional approaches, which are based on first-order statistics of images, the method uses high-order pooling to use second-order statistics to capture long-range dependencies between slices of images.

They used 833 T1-weighted MRI images from ADNI, out of which 221 are AD subjects, 297 are MCI subjects, and 315 are Normal Controls (NC) subjects. The accuracy of the method is better than \cite{li2019hybrid} and \cite{cheng2017classification} which are based on denseNets and Recurrent Neural Network, and 3D-CNNs. The visualization of MRI images generated by their model shows that it is able to learn and generate plausible images.

Mostly focussed on the method, no discussion on the interpretation of results from clinical point of view

\cite{pan2021decgan}
The paper aims to use multi-modal imaging data- Diffusion Tensor Imaging (DTI) and rs-fMRI to detect crucial neural circuits for AD. The idea is to efficiently extract complementary topology information between rs-fMRI and DTI using a decoupling deep learning model comprising GCN and GAN. The proposed model helps decouple brain networks present in the AD population from those in the healthy population. The decoupling in the model is ensured by using adversarial learning, which extracts features discriminative of the AD. To improve the robustness of the proposed model, a sparse capacity loss is applied, which characterizes the intrinsic topological difference between different brain networks. Also, It is interesting to note that even though the paper focuses on AD, it can be easily extended to other neurodegenerative disorders. 

\cite{zhao2020functional}

In the past decade, interest in analyzing synchronous patterns in the human brain has increased manifold because these patterns are believed
to reflect the patterns of interaction between neuronal populations. A set of functionally connected regions is referred to as a ``functional network''. The functional networks are usually recovered from functional connectivity. FC is defined as the correlation between blood-oxygen-level-dependent (BOLD) signals of different regions of interest extracted from resting-state functional magnetic resonance imaging (rs-fMRI).  

This work was the first attempt to apply the GAN model for disease classification using functional connectivity promising neuroimaging biomarkers. The model uses aims to discriminate MDD vs. HC and
SZ vs. HC. Functional connectivity matrices were calculated by correlation
of time courses derived from independent components. The GAN model is combined with adversarial training and feature matching for brain disease diagnosis using the FNC. They compared the proposed approach with $5$ traditional methods and the DNN approach. The model achieved $5.9\%$ higher in MDD classification and $1.8\%$ higher in SZ classification, suggesting its utility as a
potentially powerful tool to aid discriminative diagnosis.



\section{Future work}

Fairness-aware learning- This has become important in machine learning models, especially where the goal is to conduct predictive analysis. It aims at discrimination prevent so that the training model is not biased. FairGAN: Fairness-aware Generative Adversarial Networks \cite{xu2018fairgan}

Domain adaption- Very limited work in analyzing fMRI and DTI multi-site data.

Heterogeneity- Although GCNs have given impressive results in the field of human brain network analysis, learning latent embeddings faces several challenges, including heterogeneity in data and the noisy connections in brain networks.

Data shortage- Use of deep learning networks such as deep convolutional GAN (DCGAN) \cite{yi2019generative,gui2021review} can be used to address the problem of data shortage. The generation of artificial data from different classes of a disorder with GAN architectures' help can be considered the future work for effective diagnosis of this disease. Another challenge is the lack of free access to sMRI or fMRI neuroimaging modalities for a particular disorder class. Zero-shot learning can solve the problem of not having access to the data of a class \cite{wang2019survey,xian2018feature}.



